Touch2Shape: Touch-Conditioned 3D Diffusion for Shape Exploration and Reconstruction

Diffusion models have made breakthroughs in 3D generation tasks. Current 3D diffusion models focus on reconstructing target shape from images or a set of partial observations. While excelling in global context understanding, they struggle to capture the local details of complex shapes and limited to the occlusion and lighting conditions. To overcome these limitations, we utilize tactile images to capture the local 3D information and propose a Touch2Shape model, which leverages a touch-conditioned diffusion model to explore and reconstruct the target shape from touch. For shape reconstruction, we have developed a touch embedding module to condition the diffusion model in creating a compact representation and a touch shape fusion module to refine the reconstructed shape. For shape exploration, we combine the diffusion model with reinforcement learning to train a policy. This involves using the generated latent vector from the diffusion model to guide the touch exploration policy training through a novel reward design. Experiments validate the reconstruction quality thorough both qualitatively and quantitative analysis, and our touch exploration policy further boosts reconstruction performance.

==> chart/fig_failure.tex <==
%----------------------------------------------------------------------------------
\begin{figure*}[tp!]
\begin{center}
  \begin{minipage}{0.14\linewidth}
  \centering{\textbf{Ground \\ truth}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/958/mesh_gt.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/1011/mesh_gt.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/1046/mesh_gt.png}}
  \end{minipage}  
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/1264/mesh_gt.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/2624/mesh_gt.png}}
  \end{minipage}

  \begin{minipage}{0.14\linewidth}
  \centering{\textbf{points \\ (ActiveVT)}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/958/points.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/1011/points.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/1046/points.png}}
  \end{minipage}  
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/1264/points.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/2624/points.png}}
  \end{minipage}  

  \begin{minipage}{0.14\linewidth}
  \centering{\textbf{points \\ (ours)}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/sdfvt/958/points_gen.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/sdfvt/1011/points_gen.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/sdfvt/1046/points_gen.png}}
  \end{minipage}  
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/sdfvt/1264/points_gen.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/sdfvt/2624/points_gen.png}}
  \end{minipage}  

  \begin{minipage}{0.14\linewidth}
  \centering{\textbf{mesh \\ (ActiveVT)}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/958/mesh.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/1011/mesh.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/1046/mesh.png}}
  \end{minipage}  
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/1264/mesh.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/activevt/2624/mesh.png}}
  \end{minipage}  

  \begin{minipage}{0.14\linewidth}
  \centering{\textbf{mesh \\ (ours)}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/sdfvt/958/mesh_gen.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/sdfvt/1011/mesh_gen.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/sdfvt/1046/mesh_gen.png}}
  \end{minipage}  
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/sdfvt/1264/mesh_gen.png}}
  \end{minipage}
  \begin{minipage}{0.16\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/failure/sdfvt/2624/mesh_gen.png}}
  \end{minipage}  
  
  \caption{ \label{fig:fig_failure}
           Some failure cases.
           }
%  976, 649, 661, 874, 1616, 2752, 908, 4136
% failure: 958, 1011, 1037, 1046, 1264, 1480, 2624
\end{center}
\vspace{-0.4cm} 
\end{figure*}





==> chart/fig_sdft.tex <==
%----------------------------------------------------------------------------------
\begin{figure*}[tp!]
\begin{center}
  \begin{minipage}{0.12\linewidth}
  \centering{\textbf{Ground \\ truth}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/1480/mesh_gt.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/2805/mesh_gt.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/3320/mesh_gt.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/4056/mesh_gt.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/4496/mesh_gt.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/3021/mesh_gt.png}}
  \end{minipage}

  \begin{minipage}{0.12\linewidth}
  \centering{\textbf{points \\ (ActiveVT)}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/1480/points.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/2805/points.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/3320/points.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/4056/points.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/4496/points.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/3021/points.png}}
  \end{minipage}  

  \begin{minipage}{0.12\linewidth}
  \centering{\textbf{points \\ (ours)}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/1480/points_gen.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/2805/points_gen.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/3320/points_gen.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/4056/points_gen.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/4496/points_gen.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/3021/points_gen.png}}
  \end{minipage}  
  
  \begin{minipage}{0.12\linewidth}
  \centering{\textbf{mesh \\ (ActiveVT)}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/1480/mesh.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/2805/mesh.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/3320/mesh.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/4056/mesh.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/4496/mesh.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/activet5/3021/mesh.png}}
  \end{minipage}    

  \begin{minipage}{0.12\linewidth}
  \centering{\textbf{mesh \\ (ours)}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/1480/mesh_gen.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/2805/mesh_gen.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/3320/mesh_gen.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/4056/mesh_gen.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/4496/mesh_gen.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=0.8\textwidth]{fig/abc_t/sdft5/3021/mesh_gen.png}}
  \end{minipage}  

  
  \caption{ \label{fig:fig_sdft}
           Qualitative results of ActiveVT \cite{activevt} and ours under the tactile only setting (5 grasps). While ActiveVT struggles with visualizations and detail preservation, our method excels in maintaining global shape across diverse structures, and ensuring the local details.}
%  1480, 2805, 1511, 2624, 4496, 3021, 3320, 3839, 4056, 4136, 4189, 4437, 4513



\end{center}
\vspace{-0.4cm} 
\end{figure*}





==> chart/fig_shapenet.tex <==
% %------------------------------------------------------------------------
% \begin{figure*}[htbp]
%   \centering
%   \includegraphics[width=0.999\linewidth]{fig/shapenet.png}
%   \caption{\label{fig:fig_shapenet}
%          Reconstruction visualizations of seen and unseen objects on dataset ShapeNet. 
%          }


%    % train: 1a6196, 1b4d78, 1bc5d3, 7e49ef, 8da5db, 5d42d4, 5e914dd, 9db4b2, 6bb307, 7de119, 9b9349, 
%    % test: d3b53f, dad399, e81606, f93463, cda15e, d1f9e0
% % \vspace{-0.4cm} 
% \end{figure*}



%----------------------------------------------------------------------------------
\begin{figure*}[tp!]
\begin{center}

  \begin{minipage}{0.99\linewidth}
  \centering{\textbf{Seen objects and poses}}
  \end{minipage}
  

  \begin{minipage}{0.12\linewidth}
  \centering{\textbf{Ground \\ truth  \\ \vspace{30pt} Reconstructed Mesh \\ (20 touches)}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/train/1.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/train/2.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/train/3.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/train/4.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/train/5.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
 \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/train/6.png}}
  \end{minipage}

  \vspace{7.5pt}

  
  \begin{minipage}{0.99\linewidth}
  \centering{\textbf{Unseen objects and poses}}
  \end{minipage}  

  \begin{minipage}{0.12\linewidth}
  \centering{\textbf{Ground \\ truth  \\ \vspace{30pt} Reconstructed Mesh \\ (20 touches)}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/test/1.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/test/3.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/test/6.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/test/2.png}}
  \end{minipage}
  \begin{minipage}{0.14\linewidth}
  \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/test/4.png}}
  \end{minipage}  
  \begin{minipage}{0.14\linewidth}
 \centerline{\includegraphics[width=1\textwidth, height=1.6\textwidth]{fig/shapenet/test/5.png}}
  \end{minipage}
  
  \caption{ \label{fig:fig_shapenet}
           Reconstruction visualizations of seen and unseen objects on dataset ShapeNet.}
%  1480, 2805, 1511, 2624, 4496, 3021, 3320, 3839, 4056, 4136, 4189, 4437, 4513



\end{center}
\vspace{-0.4cm} 
\end{figure*}





==> chart/tab_network.tex <==
%-----------------------------------------------------------------------
\begin{table*}[htbp]
% \vspace{-2.0em}\\\
\renewcommand{\arraystretch}{1.0}
\begin{center}
\begin{tabular}{| p{3cm} | p{3cm} | p{3cm} | p{3cm} | p{3cm} |}
\hline
\textbf{\makebox[0.08\textwidth][c]{Model}} &\textbf{\makebox[0.12\textwidth][c]{Module}}  &\textbf{\makebox[0.12\textwidth][c]{Input shape}} &\textbf{\makebox[0.12\textwidth][c]{Operation}} &\textbf{\makebox[0.12\textwidth][c]{Output shape}}     \\
\hline  
\multirow{6}{*}{\makecell{\textbf{{Touch Embed}}}} &\multirow{2}{*}{\makecell{\textbf{{CNN Block 1}}}} &$20 \times 25 \times 4$  &Conv ($1 \times 1$) + BN + ReLU   &$20 \times 25 \times 128$    \\
& &$20 \times 25 \times 128$  &Conv ($1 \times 1$) + BN + ReLU   &$20 \times 25 \times 256$    \\
\cline{2-5}
&\multirow{2}{*}{\makecell{\textbf{{CNN Block 2}}}} &$20 \times 25 \times 512$  &Conv ($1 \times 1$) + BN + ReLU   &$20 \times 25 \times 1024$    \\
& &$20 \times 25 \times 1024$  &Conv ($1 \times 1$) + BN + ReLU   &$20 \times 25 \times 768$    \\
\cline{2-5}
&\multirow{2}{*}{\makecell{\textbf{{Position Embed}}}} &$20 \times 3$  &FC + ReLU   &$20 \times 128$    \\
& &$20 \times 128$  &FC   &$20 \times 768$    \\
\hline

\multirow{11}{*}{\makecell{\textbf{{Latent Encoder}}}} &\multirow{2}{*}{\makecell{\textbf{{CNN Block 1}}}} &$16 \times 16 \times 16 \times 3$  &Conv ($3 \times 3 \times 3$) + BN + ReLU   &$16 \times 16 \times 16 \times 128$    \\
& &$16 \times 16 \times 16 \times 128$  &Conv ($3 \times 3 \times 3$) + BN + ReLU   &$16 \times 16 \times 16 \times 128$    \\
& &$16 \times 16 \times 16 \times 128$  &Average Pooling ($2 \times 2 \times 2$)   &$8 \times 8 \times 8 \times 128$    \\
\cline{2-5}
&\multirow{2}{*}{\makecell{\textbf{{CNN Block 2}}}} &$8 \times 8 \times 8 \times 128$  &Conv ($3 \times 3 \times 3$) + BN + ReLU   &$8 \times 8 \times 8 \times 512$    \\
& &$8 \times 8 \times 8 \times 512$  &Conv ($3 \times 3 \times 3$) + BN + ReLU   &$8 \times 8 \times 8 \times 512$    \\
& &$8 \times 8 \times 8 \times 512$  &Average Pooling ($2 \times 2 \times 2$)   &$4 \times 4 \times 4 \times 512$    \\
\cline{2-5}
&\multirow{2}{*}{\makecell{\textbf{{CNN Block 3}}}} &$4 \times 4 \times 4 \times 512$  &Conv ($3 \times 3 \times 3$) + BN + ReLU   &$4 \times 4 \times 4 \times 512$    \\
& &$4 \times 4 \times 4 \times 512$  &Conv ($3 \times 3 \times 3$) + BN + ReLU   &$4 \times 4 \times 4 \times 512$    \\
& &$4 \times 4 \times 4 \times 512$  &Average Pooling ($2 \times 2 \times 2$)   &$2 \times 2 \times 2 \times 512$    \\
\cline{2-5}
&\multirow{2}{*}{\makecell{\textbf{{Linear Layer}}}} &$2 \times 2 \times 2 \times 512$  &Reshape   &$1 \times 4096$ \\
& &$1 \times 4096$  &FC   &$1 \times 768$    \\
\hline

\multirow{6}{*}{\makecell{\textbf{Touch Shape Fusion}}} &\multirow{3}{*}{\makecell{\textbf{{Encoder Layers}}}} &$64 \times 64 \times 64 \times 1$  &Input Convolution   &$64 \times 64 \times 64 \times 64$    \\
& &$64 \times 64 \times 64 \times 64$  &Down Block 1   &$32 \times 32 \times 32 \times 256$    \\
& &$32 \times 32 \times 32 \times 256$  &Down Block 2,3,4 + Middle Block  &$16 \times 16 \times 16 \times 256$    \\
\cline{2-5}

&\multirow{3}{*}{\makecell{\textbf{{Decoder Layers}}}} &$16 \times 16 \times 16 \times 3$  &Convolution + Middle Block  &$16 \times 16 \times 16 \times 256$    \\
& &$16 \times 16 \times 16 \times 256$  &Up Block 1   &$32 \times 32 \times 32 \times 256$    \\
& &$32 \times 32 \times 32 \times 256$  &Up Block 2,3,4  &$64 \times 64 \times 64 \times 64$    \\
\hline

\multirow{7}{*}{\makecell{\textbf{{Policy Model}}}} &\multirow{3}{*}{\makecell{\textbf{{Action Embed}}}} &$1 \times 50$  &FC + ReLU  &$1 \times 128$    \\
& &$1 \times 128$  &FC + ReLU   &$1 \times 256$    \\
& &$1 \times 256$  &FC  &$1 \times 768$    \\
\cline{2-5}

 &\multirow{4}{*}{\makecell{\textbf{{Value Net}}}} &$(1 \times 768) \times 3$  &Concatenating   &$1 \times 2304$    \\
  & &$1 \times 2304$  &FC + ReLU   &$1 \times 512$    \\
  & &$1 \times 512$  &(FC + ReLU) $\times 3$   & $1 \times 128$    \\ 
& &$1 \times 128$  &FC   &$1 \times 50$    \\
\hline

\end{tabular}
\caption{ \label{tab_network}
    Architecture of each model. Conv: convolution layers with different kernel size, BN: batch normalization layers, ReLU: Rectified Linear Unit, FC: Fully Connected layers.    
    }
\end{center}
% \vspace{-0.4cm} 
\end{table*}
%-------------------------------------------------------------------------

==> chart/tab_num_touch.tex <==

%%-----------------------------------------------------------------------
\begin{table}[htbp]
\renewcommand{\arraystretch}{1.0}
\begin{center}
\begin{tabular}{|  c | c  c c c c c|}
\hline
\multirow{2}{*}{\makecell{\textbf{\makebox[0.05\textwidth][c]{Method}}}} &\multicolumn{6}{c|}{\textbf{{Grasp \#}}} \\
\cline{2-7}
  &\makebox[0.03\textwidth][c]{0}  &\makebox[0.03\textwidth][c]{1} &\makebox[0.03\textwidth][c]{2} &\makebox[0.04\textwidth][c]{3} &\makebox[0.03\textwidth][c]{4} &\makebox[0.03\textwidth][c]{5}  \\
\hline
Oracle  &100 &12.0 &6.86 &5.01 &4.90 &4.88  \\
Random   &100 &21.9 &13.5 &10.5 &8.82 &8.14 \\
Even  &100 &15.3 &10.2 &9.13 &8.23 &7.44 \\
Ours   &100 &16.9 &9.62 &7.62 &6.88 &6.63 \\
\hline
\end{tabular}
\caption{ \label{tab_num_touch}
    Comparison of touch exploration policy on dataset ABC under touch only setting. The evaluation metric is CD error. 
} 
\end{center}
% \vspace{-0.4cm} 
\end{table}
%-------------------------------------------------------------------------



